Bidding Strategies with Gender Nondiscrimination: Constraints for Online Ad Auctions

Interactions between bids to show ads online can lead to an advertiser's ad being shown to more men than women even when the advertiser does not target towards men. We design bidding strategies that advertisers can use to avoid such emergent discrimination without having to modify the auction mechanism. We mathematically analyze the strategies to determine the additional cost to the advertiser for avoiding discrimination, proving our strategies to be optimal in some settings. We use simulations to understand other settings.

==> conclusion.tex <==
\section{Conclusion}


==> constrained_k_strict.tex <==
\section{{Scenario 3: Simple Advertiser with K-Strict Policy }}

In the previous sections, we focused on an advertiser where it is very restricted. However, the advertiser may be able to relax the constrained and instead of enforcing the difference between the number of the female and the male viewer wins to be one, it allows the difference to be up to $k$. So we define \textit{K-Strict Non-discriminatory Advertiser} as follow:


\begin{definition}{\textbf{K-Strict Non-discriminatory Advertiser}}
An advertiser is a K-strict non-discriminatory when at each round of auction the maximum of difference between the number of auctions that it wins for each user type is $K$.
\end{definition}

\par Similar to the previous scenario, we each advertiser has a limited budget $B_n$ and it uses i.i.d bidding strategy from a fixed distribution $F_n$. In this scenario, we will re-use all of the estimations from section~\ref{sec:strict_constrained}.

\subsection{Baseline}
The unrestricted advertiser in this scenario is the equivalent of the advertiser from the previous section. Therefore we use the same utility functions from section~\ref{ssec:strict_constraint_unrestricted} for the budget constrained advertiser and section~\ref{ssec:strict_unconstraint_unrestricted} for the unconstrained budget case. 
\subsection{Restricted Advertiser}



 
\begin{algorithm}[t]
    \SetAlgoNoLine
    $WM$ = 0; 

        \For{each auction $t$ }{
            
            \If{ ( $-K<WM <K$ ) }{
                Participate auction at $t$\;
            }
           \If{($WM == -K$) \text{and} ($\theta^t == Male$)}
           {
           Participate auction at $t$\;
           }
           \If{($WM==K$) \text{and} ($\theta^t == Female$)}
           {
           Participate auction at $t$\;
           }
           \If{\textup{Participate} \text{and} ($d_g^t \leq b_g^t$)}{
                
                    \eIf{$\theta^t == Male$}{
                        $WM$ += 1;
                    }
                    {
                        $WM$ -= 1;
                    }
                }
            
        }
        
    \caption{Mechanism for K-strict advertiser}
    \label{alg:k-strict}
\end{algorithm}

Algorithm~\ref{alg:k-strict} is a modified version algorithm~\ref{alg:strict} to allow up to $K$ difference between the number of wins for the male and female viewer. In section~\ref{sec:k-optimality} we prove the optimality of this algorithm for the K-strict advertiser.


\begin{figure}
\centering
\includegraphics[scale=0.6]{{k_strict_MC}}
\caption{Markov chain model for a K-strict non-discriminatory screening algorithm}
\label{fig:mc_kstrict}
\end{figure}


\begin{figure}
\centering
\includegraphics[scale=0.3]{{Kstrict_diff_p}}
\caption{The impact of different gender distribution on the utility}
\label{fig:kstrict}
\end{figure}

\par Similar to the algorithm~\ref{alg:strict}, we modeled the behavior of the algorithm using a Markov chain (see figure~\ref{fig:mc_kstrict}) and computed the stationary distribution for the Markov model. 
The probability of the participating in an ad slot auction in the steady state is as follow:
\begin{align}
 \frac{2 p (1-p) (1- (\frac{p}{1 - p})^{2k})}{1 - p (1+  (\frac{p}{1 - p})^{2k})}
\end{align}

\par So we can replace the probability of participating from the previous scenarios by the above equation, to find the cost of the K-strict non-discriminatory advertiser. Therefore, for the unlimited budget advertiser the cost of  K-strict non-discriminatory is:
\begin{align}
E[U'_g]=|W|\frac{2 p (1-p) (1- (\frac{p}{1 - p})^{2k})}{1 - p (1+  (\frac{p}{1 - p})^{2k})} \mu_g 
\end{align}
If the budget of unrestricted advertiser does not finish by the round $T$ the cost using K-strict non-discriminatory advertiser is similar to the unlimited budget case which is the same value as above.

In the case the unrestricted advertiser finishes the its budget at round $\tau_g$ which is less than $T$ and the restricted advertiser does not finishes the budget. We can rewrite equation ~\ref{eq:strict_notfinish_budget} when we do not have discounting factor as follow:
\begin{align}
E[U'_g] \geq \left(\frac{T}{\tau_g} \times \frac{2 p (1-p) (1- (\frac{p}{1 - p})^{2k})}{1 - p (1+  (\frac{p}{1 - p})^{2k})} |W|  \right) \times \mu_g
\end{align}
And for the discounted case as :
\begin{align}
E[U'_g]\geq \left((\frac{1-\delta^{T-\tau_g}}{1-\delta})  \times (\frac{T}{\tau_g}) \times (\frac{2 p (1-p) (1- (\frac{p}{1 - p})^{2k})}{1 - p (1+  (\frac{p}{1 - p})^{2k})} |W|)  \right) \times \mu_g
\end{align}

To demonstrate the effect of $K$ on the cost for the advertiser $g$ we plotted the ratio of utility for the restricted and unrestricted advertisers in figure~\ref{fig:kstrict}. As we can observe, when the male and the female viewers population are unbalanced, increasing $K$ will not increase the lower bound of the utility of the restricted advertiser. This is due to the fact that in a steady state regime if for example men are more than women, the screening algorithm will always have enough men to chose and end up in the state where it has $K$ more men than women. As a result the $K$ does not have have huge impact on the steady state and only it determine how much it does take to reach to the steady state. If $K$ is in order of the $T$ the Markov model may not reach the steady state at all and the probability of the participating will be higher than the steady state analysis. However, In the real-world scenarios $K$ is much smaller than $T$.
\subsection{On Optimality of Algorithm~\ref{alg:k-strict}}\label{sec:k-optimality}

We prove the algorithm~\ref{alg:k-strict} is optimal for all $K$ by using  induction method. 
\par \textit{Base case:} When $K$ is one the algorithm reduces to the algorithm~\ref{alg:strict} and we proved in section~\ref{sec:optimality} the optimal of this case. 

\par \textit{Induction hypothesis:} Let's assume algorithm~\ref{alg:k-strict} is optimal when $K=\kappa$ and has the highest participation probability among all algorithms. 
\par \textit{Induction step:} We need to show the algorithm~\ref{alg:k-strict} is optimal when $K=\kappa +1$. There two cases for the difference between two gender either it never goes from $\kappa $ to $\kappa+1$, therefore we know from the hypothesis algorithm~\ref{alg:k-strict} is optimal in that case. Without loss of generality, when the difference male and female viewer is $\kappa$ and one more men viewer arrives we assume there is an alternative algorithm with participate in the ad slot for the viewer with probability $\alpha$ and do not participate it probability $1-\alpha$, similar the case in section~\ref{sec:optimality} it is easy to see the over all probability of participating in all auction will be at it maximum when $\alpha$ is one. Hence, algorithm~\ref{alg:k-strict} is optimal for all $K$.   \qed


==> constrained_strict.tex <==

\section{Scenario 2: Simple Budget Constrained Advertiser with Strict Policy }\label{sec:strict_constrained}

Due to cash flow issues, advertisers may have a finite budget and be
unable to bid on slots even if the slots would have positive utility
and be worth their cost.
In this scenario, each advertiser $n$ has a limited budget of $B_n$.
Most ad exchanges let advertisers specify such a budget per day or week.
The exchanges allow the advertisers participate in ad slot auctions as
long as their budget is not yet exhuested.

In this scenario, the value of each ad slot at auction is similar to
the previous scenario.
The advertiser can only use the i.i.d.\@ bidding strategy.\mct{why?}
% Similar the previous settings, we assume each advertiser bids
% truthfully and each bid is independently drawn from a distribution
% $F_n$.
Unlike the previous setting bidding truthfully is not the optimal
strategy for even advertisers without a parity constraint~\cite{}.
Intutively, such an advertiser should skip ads with modestly positive
utility but a high second hightest bid since they will exhusest the
budget preventing the advertiser from bidding on later ads with a high
positive utility and modest second highest bid.
Despite this simple intuition, the optimal bidding strategy for this
setting is still unknown~\cite{}.

Moreover, most advertisement platforms only allow for a fixed bidding
strategy.
Therefore, we can model the problem using an i.i.d.\@
distribution.
\mct{Can we get rid of this?}

Similar to the previous scenario we first analyze the advertiser in an
unrestricted setting and then compare the results to the restricted
advertiser.


\subsection{Baseline}\label{ssec:strict_constraint_unrestricted}

Let's consider a specific advertiser $n$ who has a limited budget
$B_n$. At every round of ad slot auction advertiser, $n$ will submit
its bids according to distribution $F_n$. The advertiser keeps bidding
on the ad slot auctions as long as it has enough credit. Similar the
previous scenario the advertiser will win a set of auctions which we
indicate by $W$. The total utility of the advertiser can be computed
using equation~\eqref{eq:utility}. Since the advertiser has a limited
budget, it may not have enough budget to participate in all $T$ ad
slot auctions. We indicate the last ad slot auction round which the
advertiser $n$ participated on by $\tau_n$ which is less or equal than
$T$.

\mct{How does this model holding back?}


\subsection{Restricted Advertiser}

Similar to the restricted advertiser in the first scenario.
Each restricted advertiser should use a screening algorithm to make
sure the restriction of the non-discriminatory advertising is not
violated.
Since the bidding and the value for the each ad slot auction is
similar the previous scenario the algorithm~\ref{alg:strict} is
optimal in this scenario as well.
\mct{proof?}
To analyze the effect of the non-discriminatory advertising for a
budget constrained advertiser. Let focus on a specific advertiser $n$
and compute its utility in this setting and compare to the baseline.

The restricted advertiser $n$ will use algorithm~\ref{alg:strict} to
make sure at each moment of time he can have the same number of men
and women (give or take one).
Let's assume that the advertiser has a large budget and cannot spend
all of it in before the auctions end.
In this case $\tau_n$ is $T$, which is similar to not having any
budget constraint.
Thus, we can use the results from the previous scenario.

Next, let's assume our advertiser $n$ can use all of its budget before
round $T$, so that $\tau_n$ is strictly less than $T$.

\begin{corollary}
The maximum loss of applying a parity restriction to budget
constrained advertiser is $\frac{2p(1-p)}{1-p(1-p)}$ where $p$ is
the ratio of the two types of webpage visitors.
\end{corollary}
\begin{proof}
For any value of $\tau_n$ and distributions of the bids, if the
restricted advertiser $n$ follows Algorithm~\ref{alg:strict} until
round $\tau_g$ and does not participate to any other ad
auctions. The problem converts to the case where $\tau_n = T$, and
is similar to the previous case loss is a factor of
$\frac{2p(1-p)}{1-p(1-p)}$.
\end{proof}
\mct{I don't know what the ``maximum'' is over.}

We saw the maximum loss of applying such restriction.
However, if the restricted advertiser $n$ keeps participating in ad
slot auctions after round $\tau_n$ according to
Algorithm~\ref{alg:strict} it may win other auction which increases
its utility.

There are two possible outcomes.
Either, the advertiser $n$ finishes it budget before reaching the end
of ad slot auction rounds or it finishes the auction rounds without
running out of the budget.
\mct{repeated from above.}
In the first case, if we assume the budget of the other advertisers is
unlimited (or not finished by round $\tau_n$)\mct{why is this valid?},
then there exist fixed distributions $D_1$ and $D_2$ (as a function of
advertisers' bid distributions) such that the first bid and the second
bid are i.i.d.\@ samples from $D_1$ and $D_2$,
However, if some of the advertisers run out of the budget the
distribution of the $D_1$ and $D_2$ will change as they run out.
However, it is easy to see that
 \begin{align}
  \max_{1\leq n' \leq N} b^t_{n'} \geq \max_{1\leq n' \leq N-1} b^t_{n'} 
 \end{align}
Thus, if we indicate the distribution of the first and second bid for
each round by $D^t_1$ and $D^t_2$. We have $D^t_1 \geq D^{t+1}_1$ and
$D^t_2 \geq D^{t+1}_2$.
Therefore, the expected utility of the advertiser $n$ at each round
$t+1$ is greater or equal than the expected utility at round $t$.
For the same reason, the number of auctions a restricted version of
advertiser $n$ would win is greater or equal to the number an
unrestricted version of advertiser $n$ would win.
As a result, given an i.i.d.\@ (or fixed) bidding strategy the utility
of the restricted advertiser $n$ is at least the utility of the
unrestricted advertiser.
\mct{Assuming it gets to spend it whole budget?}
We denote the mean of utility for the restricted advertiser by
$\mu_n$.\mct{not used}
The price the restricted advertiser pays is the delay in the getting
to this same level of utility since the unrestricted advertiser can
get the same utility in a shorter time.

To analyze the second outcome where the budget of the unrestricted
advertiser finishes before $T$ rounds.
We have to find out how many auctions restricted advertiser $n$ will
win from rounds $\tau_n$ to $T$.

We can estimate the probability of winning an auction for advertiser
$n$.
To do that we can use the maximum likelihood estimation method.
In particular, we can use the Bernoulli distribution to model winning
in each round.
So we can estimate the probability of winning as
\begin{align}
P(b_n^t\geq \max_{i \in N} b_i^t ) \approx \frac{|W|}{\tau_n}
\end{align}
Similar the case since all advertisers has a limited budget, the probability of the winning for the advertiser g in round $t+1$ is greater or equal than round $t$.  
We can estimate the probability of participating and wining for each ad slot auction from $\tau_n$ to $T$ for the restricted advertiser $n$ as the product of winning an ad slot auction and the probability of participating on that auction:
\begin{align}
P(b_n^t\geq \max_{n' \in N} b_{n'}^t \ and \ ||Men|-|Women|| \leq 1) \geq \frac{|W|}{\tau_n} \times \frac{2p(1-p)}{1-p(1-p)}
\end{align}

We can compute the expected number of wining auctions in from round $\tau_g$ to $T$ as follow:
\begin{align}
\E[W'_{\tau_n,T}]  =  (T-\tau_n) \times \frac{|W|}{\tau_n} \times \frac{2p(1-p)}{1-p(1-p)}
\end{align}
So the expected total utility of the restricted advertiser is
\begin{align}
\E[U'_n] =& \sum_{t=1}^T P(participate\ at\ t,Winning\ at\ t)\times u_n \nonumber \\
=& \sum_{t \in W} P(participate\ at\ t )\times u_n \nonumber \\
  &+ \sum_{t=\tau_n}^T  P(participate\ at\ t,Winning\ at\ t)\times u_n \nonumber \\
 \geq & \left( \frac{2p(1-p)}{1-p(1-p)} |W|  + \left( (T-\tau_n) \frac{|W|}{\tau_n} \times \frac{2p(1-p)}{1-p(1-p)} \right) \right) \times \E[u_n] \nonumber\\
=& \left(\frac{T}{\tau_n} \times \frac{2p(1-p)}{1-p(1-p)} |W|  \right) \times \mu_n \label{eq:strict_notfinish_budget}
\end{align}

So  applying restriction on simple budget constrained advertiser $n$ will reduce the expected total utility of the advertiser by at most a factor of $\min(\frac{T}{\tau_n} \times \frac{2p(1-p)}{1-p(1-p)},1)$.

The general result of our analysis shows that the restricted the restricted advertisers should wait for more to get the similar number of users. Specifically, we can compute the upper bound on $T$ such that the expected total utility remains the same. 
\begin{align}
T_{min} \leq \tau_n \frac{1-p(1-p)}{2p(1-p)}
\end{align}

So if the restricted advertiser $n$ waits on average $\frac{1-p(1-p)}{2p(1-p)}$ more that unrestricted, he can gain the similar benefit.


\subsection{Discounting}

The time span of an online ad is usually limited. For example, a specific online ad may only be advertised for a week or month. However, for the cases when the time span in higher, we may want to consider a discounting factor in the utility functions. In this case, the bidding strategy stays the same (as explained before) and we want to compare the discounted utility of the restricted advertise to the unrestricted. Let us indicate the discount factor by $\delta$. Therefore we can rewrite the utility of the advertiser as follow: 
\begin{align}
\E[U'_n]=& \sum_{t \in W} P(participate\ at\ t ) \times u_n \nonumber \\
& + \sum_{t=\tau_n}^T \delta^{t-\tau_n}  P(participate\ at\ t,Winning\ at\ t)\times u_n  \nonumber \\
  \geq & \left( \frac{2p(1-p)}{1-p(1-p)} |W|  + \left((\frac{1-\delta^{T-\tau_n}}{1-\delta}) (T-\tau_n) \frac{|W|}{\tau_n}  \right. \right. \nonumber \\
  & \left. \left. \times \frac{2p(1-p)}{1-p(1-p)} \right) \right) \times \E[u_n] \nonumber \\
=& \left((\frac{1-\delta^{T-\tau_n}}{1-\delta})  \times (\frac{T}{\tau_n}) \times (\frac{2p(1-p)}{1-p(1-p)} |W|)  \right) \times \mu_n
\end{align}
 
When we use a discounted utility function the restricted advertiser's expected total utility value reduces by a factor of $(\frac{1-\delta^{T-\tau_n}}{1-\delta})  \times (\frac{T}{\tau_n}) \times (\frac{2p(1-p)}{1-p(1-p)})$, for the cases the where budget does not finishes by the end of the end of the ad slot auction rounds. and $(\frac{1-\delta^{ \tau_n \frac{1-3p(1-p)}{2p(1-p)}}}{1-\delta})$ when  use all of the budget before round $T$.


==> mechanism.tex <==
\section{Mechanism}






\begin{algorithm}[t]
        \SetAlgoLined
\DontPrintSemicolon

\KwIn{$V,\kappa,\theta^*,K$}
    \SetKwFunction{FMain}{$K$-strict Bidding}
    \SetKwProg{Fn}{Function}{:}{}
    \Fn{\FMain{$V,\kappa,\theta^*,K$}}{
        {\If{$\kappa=K$ and $\theta^*=1$}{
        \textbf{return} $0 $ 
        
        }}
        {\If{$\kappa=-K$ and $\theta^*=0$}{
        \textbf{return} $0 $ 
        
        }}
        {\eIf {$\theta^*=1$}{
        \textbf{return} $\Gamma^m(\kappa)$
        }{
        \textbf{return} $\Gamma^w(\kappa)$
        }}

        
}
\textbf{End Function}      
    \caption{Bidding mechanism for K-strict advertiser}
    \label{alg:k-strict}
\end{algorithm}

 
\begin{algorithm}[t]
        \SetAlgoLined
\DontPrintSemicolon

\KwIn{$g^m,g^w,\alpha,v^m,v^w,\epsilon$}
    {\textbf{Initialize} $V[-K:K,0:1]=\frac{v^m+v^w}{2}$}
    
        {\Repeat{$\Delta>\epsilon$}{
        {$\Delta \gets 0$}
        
        {\For{$k\gets -K$ to $K$}
        {
        {$V^*[k,1] \gets R^m(\Gamma^m(k);g_i^m)+ \delta N^m(\Gamma^m(k),k;g_i^m,g_i^w) $}
        {$\Delta= \max(\Delta,|V^*[k,1]-V[k,1]|)$}
        {$V^*[k,0] \gets R^w(\Gamma^w(k);g_i^w)+ \delta N^w(\Gamma^w(k),k;g_i^m,g_i^w) $}
        {$\Delta= \max(\Delta,|V^*[k,0]-V[k,0]|)$}
        }}
        {$V=V^*$}
        }}
        
  
    \caption{Iterative approach to find $V$}
    \label{alg:converge}
\end{algorithm}



We defined the optimal bidding strategy in the previous section. Next, we develop the bidding algorithm for the $K$-strict advertiser. Algorithm~\ref{alg:k-strict} will ensure the advertiser will bid optimally and also never violate the definition of the $K$-strict advertiser. However, we need to find value functions. To find the value functions we use algorithm~\ref{alg:converge} to iteratively converge to state values. Although, showing the convergence in general for is an open problem, we find computationally that it converges within tolerance in a feasible number of iterations.



==> method.tex <==
\section{Methodology}
 We want to design a general model which can be applied to any auction mechanism. To do so, instead of changing the auction mechanism we use a two-step auction. As we mentioned earlier, the advertisement platform will run an auction for each ad slot, and advertisers submit their bids for that ad slot. We introduce a new step. Every advertiser can have a screening phase where they get some information about the ad slot viewer and decide if they want to participate at that auction. If the advertiser decides that it wants to participate in that ad slot auction based on the viewer properties, then it submits its bids. Keep in mind that all of these processes are happening virtually which means that the advertisement platform runs the decision algorithm on behalf of the advertisers. Hence, there is no privacy leakage by providing information about the ad viewer.
 

 
\par Our goal is to design an screening algorithm which can guarantee nondiscriminatory properties independent of the advertisement platform processes.
 
\par Having the screening process has several benefits over changing to the whole advertisement platform auction method. First, it can be applied to any existing trained model, and large advertisement companies do not need change any significant model, and they easily can apply such techniques to make sure that their even if their algorithms have implicit discrimination the screening process guarantees the nondiscriminatory outcome. Moreover, not all of the advertisers are obligated to the nondiscrimination laws. Therefore, advertisement platforms can apply the screening process only to the advertisers who need this feature which can incentivize the platforms to implement this method.
